A Verified Implementation of B+-Trees in Isabelle/HOL

In this paper we present the verification of an imperative implementation of the ubiquitous B+-tree data structure in the interactive theorem prover Isabelle/HOL. The implementation supports membership test, insertion and range queries with efficient binary search for intra-node navigation. The imperative implementation is verified in two steps: an abstract set interface is refined to an executable but inefficient purely functional implementation which is further refined to the efficient imperative implementation.

==> ictac2022-bplustrees <==
@book{latex,
  title = {LaTeX : A Documentation Preparation System User's Guide and Reference Manual},
  publisher = {Addison-Wesley Professional},
  year = {1994},
  author = {Leslie Lamport}
}
@article{DBLP:journals/acta/BayerM72,
  author    = {Rudolf Bayer and
               Edward M. McCreight},
  title     = {Organization and Maintenance of Large Ordered Indices},
  journal   = {Acta Informatica},
  volume    = {1},
  pages     = {173--189},
  year      = {1972},
  url       = {https://doi.org/10.1007/BF00288683},
  doi       = {10.1007/BF00288683},
  timestamp = {Sun, 21 Jun 2020 17:37:55 +0200},
  biburl    = {https://dblp.org/rec/journals/acta/BayerM72.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@book{DBLP:books/daglib/0095349_mod,
  author    = {Michael J. Folk and
               Bill Zoellick and
               Greg Riccardi},
  title     = {File structures - an object-oriented approach with {C++}},
  publisher = {Addison-Wesley-Longman},
  year      = {1992},
  isbn      = {0-201-55713-4},
}
@book{DBLP:books/lib/Knuth98a,
  author    = {Donald Ervin Knuth},
  title     = {The art of computer programming, , Volume III, 2nd Edition},
  publisher = {Addison-Wesley},
  year      = {1998},
  url       = {https://www.worldcat.org/oclc/312994415},
  isbn      = {0201896850},
  timestamp = {Fri, 17 Jul 2020 16:12:39 +0200},
  biburl    = {https://dblp.org/rec/books/lib/Knuth98a.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{DBLP:journals/sosym/ErnstSR15,
  author    = {Gidon Ernst and
               Gerhard Schellhorn and
               Wolfgang Reif},
  title     = {Verification of B\({}^{\mbox{+}}\) trees by integration of shape analysis
               and interactive theorem proving},
  journal   = {Softw. Syst. Model.},
  volume    = {14},
  number    = {1},
  pages     = {27--44},
  year      = {2015},
  url       = {https://doi.org/10.1007/s10270-013-0320-1},
  doi       = {10.1007/s10270-013-0320-1},
  timestamp = {Mon, 26 Oct 2020 08:48:57 +0100},
  biburl    = {https://dblp.org/rec/journals/sosym/ErnstSR15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/popl/MalechaMSW10,
  author    = {J. Gregory Malecha and
               Greg Morrisett and
               Avraham Shinnar and
               Ryan Wisnesky},
  editor    = {Manuel V. Hermenegildo and
               Jens Palsberg},
  title     = {Toward a verified relational database management system},
  booktitle = {Proceedings of the 37th {ACM} {SIGPLAN-SIGACT} Symposium on Principles
               of Programming Languages, {POPL} 2010, Madrid, Spain, January 17-23,
               2010},
  pages     = {237--248},
  publisher = {{ACM}},
  year      = {2010},
  url       = {https://doi.org/10.1145/1706299.1706329},
  doi       = {10.1145/1706299.1706329},
  timestamp = {Tue, 06 Nov 2018 11:07:43 +0100},
  biburl    = {https://dblp.org/rec/conf/popl/MalechaMSW10.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@techreport{Fielding80,
  title = {The Specification of Abstract Mappings and their Implementation as B+ Trees},
  author = {Elizabeth Fielding},
  year = "1980",
  institution = "OUCL",
  month = "9",
  number = "PRG18",
  pages = "78",
}
@inproceedings{DBLP:conf/itp/Nipkow16,
  author    = {Tobias Nipkow},
  editor    = {Jasmin Christian Blanchette and
               Stephan Merz},
  title     = {Automatic Functional Correctness Proofs for Functional Search Trees},
  booktitle = {Interactive Theorem Proving - 7th International Conference, {ITP}
               2016, Nancy, France, August 22-25, 2016, Proceedings},
  series    = {Lecture Notes in Computer Science},
  volume    = {9807},
  pages     = {307--322},
  publisher = {Springer},
  year      = {2016},
  url       = {https://doi.org/10.1007/978-3-319-43144-4\_19},
  doi       = {10.1007/978-3-319-43144-4\_19},
  timestamp = {Wed, 25 Sep 2019 18:17:56 +0200},
  biburl    = {https://dblp.org/rec/conf/itp/Nipkow16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{DBLP:journals/jar/Lammich19,
  author    = {Peter Lammich},
  title     = {Refinement to Imperative {HOL}},
  journal   = {J. Autom. Reason.},
  volume    = {62},
  number    = {4},
  pages     = {481--503},
  year      = {2019},
  url       = {https://doi.org/10.1007/s10817-017-9437-1},
  doi       = {10.1007/s10817-017-9437-1},
  timestamp = {Wed, 02 Sep 2020 13:29:45 +0200},
  biburl    = {https://dblp.org/rec/journals/jar/Lammich19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{DBLP:journals/csedu/Montague91,
  author    = {Patricia T. Montague},
  title     = {A Correctness Proof for Binary Search},
  journal   = {Comput. Sci. Educ.},
  volume    = {2},
  number    = {1},
  pages     = {81--89},
  year      = {1991},
  url       = {https://doi.org/10.1080/0899340910020106},
  doi       = {10.1080/0899340910020106},
  timestamp = {Mon, 08 Jun 2020 22:36:38 +0200},
  biburl    = {https://dblp.org/rec/journals/csedu/Montague91.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@book{DBLP:books/sp/NipkowPW02,
  author    = {Tobias Nipkow and
               Lawrence C. Paulson and
               Markus Wenzel},
  title     = {Isabelle/HOL - {A} Proof Assistant for Higher-Order Logic},
  series    = {Lecture Notes in Computer Science},
  volume    = {2283},
  publisher = {Springer},
  year      = {2002},
  url       = {https://doi.org/10.1007/3-540-45949-9},
  doi       = {10.1007/3-540-45949-9},
  isbn      = {3-540-43376-7},
  timestamp = {Tue, 14 May 2019 10:00:35 +0200},
  biburl    = {https://dblp.org/rec/books/sp/NipkowPW02.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:journals/entcs/SextonT08,
  author    = {Alan P. Sexton and
               Hayo Thielecke},
  editor    = {Andrej Bauer and
               Michael W. Mislove},
  title     = {Reasoning about {B+} Trees with Operational Semantics and Separation
               Logic},
  booktitle = {Proceedings of the 24th Conference on the Mathematical Foundations
               of Programming Semantics, {MFPS} 2008, Philadelphia, PA, USA, May
               22-25, 2008},
  series    = {Electronic Notes in Theoretical Computer Science},
  volume    = {218},
  pages     = {355--369},
  publisher = {Elsevier},
  year      = {2008},
  url       = {https://doi.org/10.1016/j.entcs.2008.10.021},
  doi       = {10.1016/j.entcs.2008.10.021},
  timestamp = {Mon, 13 Jan 2020 15:55:13 +0100},
  biburl    = {https://dblp.org/rec/journals/entcs/SextonT08.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{DBLP:journals/csur/Comer79,
  author    = {Douglas Comer},
  title     = {The Ubiquitous B-Tree},
  journal   = {{ACM} Comput. Surv.},
  volume    = {11},
  number    = {2},
  pages     = {121--137},
  year      = {1979},
  url       = {https://doi.org/10.1145/356770.356776},
  doi       = {10.1145/356770.356776},
  timestamp = {Wed, 14 Nov 2018 10:31:47 +0100},
  biburl    = {https://dblp.org/rec/journals/csur/Comer79.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@techreport{OderskyScala,
author = {Odersky, Martin and Altherr, Philippe and Cremet, Vincent and Dragos, Iulian and Dubochet, Gilles and Emir, Burak and McDirmid, Sean and Micheloud, Stéphane and Mihaylov, Nikolay and Schinz, Michel and Spoon, Lex and Stenman, Erik and Zenger, Matthias},
year = {2015},
month = {03},
pages = {},
title = {An Overview of the Scala Programming Language (2. Edition)}
}
@book{DBLP:books/daglib/0069232,
  author    = {Robin Milner and
               Mads Tofte and
               Robert Harper},
  title     = {Definition of standard {ML}},
  publisher = {{MIT} Press},
  year      = {1990},
  isbn      = {978-0-262-63132-7},
  timestamp = {Tue, 14 Mar 2017 11:56:49 +0100},
  biburl    = {https://dblp.org/rec/books/daglib/0069232.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@MISC{Haftmann20codegeneration,
    author = {Florian Haftmann and Lukas Bulwahn},
    title = {Code generation from Isabelle/HOL theories},
    year = {2020}
}
@book{DBLP:books/daglib/0023376,
  author    = {Thomas H. Cormen and
               Charles E. Leiserson and
               Ronald L. Rivest and
               Clifford Stein},
  title     = {Introduction to Algorithms, 3rd Edition},
  publisher = {{MIT} Press},
  year      = {2009},
  url       = {http://mitpress.mit.edu/books/introduction-algorithms},
  isbn      = {978-0-262-03384-8},
  timestamp = {Mon, 17 Aug 2020 11:36:12 +0200},
  biburl    = {https://dblp.org/rec/books/daglib/0023376.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/lics/Reynolds02,
  author    = {John C. Reynolds},
  title     = {Separation Logic: {A} Logic for Shared Mutable Data Structures},
  booktitle = {17th {IEEE} Symposium on Logic in Computer Science {(LICS} 2002),
               22-25 July 2002, Copenhagen, Denmark, Proceedings},
  pages     = {55--74},
  publisher = {{IEEE} Computer Society},
  year      = {2002},
  url       = {https://doi.org/10.1109/LICS.2002.1029817},
  doi       = {10.1109/LICS.2002.1029817},
  timestamp = {Wed, 16 Oct 2019 14:14:54 +0200},
  biburl    = {https://dblp.org/rec/conf/lics/Reynolds02.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@book{DBLP:books/sp/NipkowK14,
  author    = {Tobias Nipkow and
               Gerwin Klein},
  title     = {Concrete Semantics - With Isabelle/HOL},
  publisher = {Springer},
  year      = {2014},
  url       = {https://doi.org/10.1007/978-3-319-10542-0},
  doi       = {10.1007/978-3-319-10542-0},
  isbn      = {978-3-319-10541-3},
  timestamp = {Fri, 02 Nov 2018 09:27:06 +0100},
  biburl    = {https://dblp.org/rec/books/sp/NipkowK14.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@manual{isabelleManual,
  title        = {The Isabelle/Isar Reference Manual},
  author       = {Makarius Wenzel},
  year      = {2020},
  url       = {https://isabelle.in.tum.de/doc/isar-ref.pdf},
}
@manual{isabelleDatatypeManual,
  title        = {Defining (Co)datatypes and Primitively(Co)recursive Functions in Isabelle/HOL},
  author       = {Julian Biendarra and Jasmin Blanchette and Martin Desharnais and Lorenz Panny and Andrei Popescu and Dmitriy Traytel},
  year      = {2020},
  url      = {https://isabelle.in.tum.de/dist/doc/datatypes.pdf}
}
@misc{MuendlerAppendix21,
    author={Niels M\"undler},
    title={A Verified Imperative Implementation of B-Trees: Appendix},
    year= {2021},
    publisher = {GitHub},
    howpublished = {\url{https://github.com/nielstron/btrees}}
}
@inproceedings{DBLP:conf/itp/Krauss10,
  author    = {Alexander Krauss},
  editor    = {Ekaterina Komendantskaya and
               Ana Bove and
               Milad Niqui},
  title     = {Recursive Definitions of Monadic Functions},
  booktitle = {Partiality and Recursion in Interactive Theorem Provers, PAR@ITP 2010,
               Edinburgh, UK, July 15, 2010},
  series    = {EPiC Series},
  volume    = {5},
  pages     = {1--13},
  publisher = {EasyChair},
  year      = {2010},
  url       = {https://easychair.org/publications/paper/hcw},
  timestamp = {Wed, 27 May 2020 16:02:35 +0200},
  biburl    = {https://dblp.org/rec/conf/itp/Krauss10.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@INPROCEEDINGS{Haftmann07acode,
    author = {Florian Haftmann and Tobias Nipkow},
    title = {A code generator framework for Isabelle/HOL},
    booktitle = {Department of Computer Science, University of Kaiserslautern},
    year = {2007}
}
@inproceedings{DBLP:conf/tphol/BulwahnKHEM08,
  author    = {Lukas Bulwahn and
               Alexander Krauss and
               Florian Haftmann and
               Levent Erk{\"{o}}k and
               John Matthews},
  editor    = {Otmane A{\"{\i}}t Mohamed and
               C{\'{e}}sar A. Mu{\~{n}}oz and
               Sofi{\`{e}}ne Tahar},
  title     = {Imperative Functional Programming with Isabelle/HOL},
  booktitle = {Theorem Proving in Higher Order Logics, 21st International Conference,
               TPHOLs 2008, Montreal, Canada, August 18-21, 2008. Proceedings},
  series    = {Lecture Notes in Computer Science},
  volume    = {5170},
  pages     = {134--149},
  publisher = {Springer},
  year      = {2008},
  url       = {https://doi.org/10.1007/978-3-540-71067-7\_14},
  doi       = {10.1007/978-3-540-71067-7\_14},
  timestamp = {Tue, 14 May 2019 10:00:48 +0200},
  biburl    = {https://dblp.org/rec/conf/tphol/BulwahnKHEM08.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{DBLP:conf/itp/Lammich19,
  author    = {Peter Lammich},
  editor    = {John Harrison and
               John O'Leary and
               Andrew Tolmach},
  title     = {Generating Verified {LLVM} from Isabelle/HOL},
  booktitle = {10th International Conference on Interactive Theorem Proving, {ITP}
               2019, September 9-12, 2019, Portland, OR, {USA}},
  series    = {LIPIcs},
  volume    = {141},
  pages     = {22:1--22:19},
  publisher = {Schloss Dagstuhl - Leibniz-Zentrum f{\"{u}}r Informatik},
  year      = {2019},
  url       = {https://doi.org/10.4230/LIPIcs.ITP.2019.22},
  doi       = {10.4230/LIPIcs.ITP.2019.22},
  timestamp = {Sat, 07 Sep 2019 02:31:13 +0200},
  biburl    = {https://dblp.org/rec/conf/itp/Lammich19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/afp/Mundler21,
  author    = {Niels M{\"{u}}ndler},
  title     = {A Verified Imperative Implementation of {B}-Trees},
  journal   = {Arch. Formal Proofs},
  volume    = {2021},
  year      = {2021},
  url       = {https://www.isa-afp.org/entries/BTree.html},
  timestamp = {Wed, 24 Mar 2021 17:37:24 +0100},
  biburl    = {https://dblp.org/rec/journals/afp/Mundler21.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/ftdb/Graefe11,
  author    = {Goetz Graefe},
  title     = {Modern B-Tree Techniques},
  journal   = {Found. Trends Databases},
  volume    = {3},
  number    = {4},
  pages     = {203--402},
  year      = {2011},
  url       = {https://doi.org/10.1561/1900000028},
  doi       = {10.1561/1900000028},
  timestamp = {Sat, 25 Apr 2020 14:00:54 +0200},
  biburl    = {https://dblp.org/rec/journals/ftdb/Graefe11.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{DBLP:journals/afp/LammichM12,
  author    = {Peter Lammich and
               Rene Meis},
  title     = {A Separation Logic Framework for Imperative {HOL}},
  journal   = {Arch. Formal Proofs},
  volume    = {2012},
  year      = {2012},
  url       = {https://www.isa-afp.org/entries/Separation\_Logic\_Imperative\_HOL.shtml},
  timestamp = {Mon, 25 May 2020 09:13:17 +0200},
  biburl    = {https://dblp.org/rec/journals/afp/LammichM12.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@misc{MuendlerAppendix22,
    author={Niels M\"undler},
    title={A Verified Imperative Implementation of {B+}-Trees: Appendix},
    year= {2022},
    publisher = {GitHub},
    howpublished = {\url{https://github.com/nielstron/bplustrees}}
}
@article{DBLP:journals/toplas/SagivRW02,
  author    = {Shmuel Sagiv and
               Thomas W. Reps and
               Reinhard Wilhelm},
  title     = {Parametric shape analysis via 3-valued logic},
  journal   = {{ACM} Trans. Program. Lang. Syst.},
  volume    = {24},
  number    = {3},
  pages     = {217--298},
  year      = {2002},
  url       = {https://doi.org/10.1145/514188.514190},
  doi       = {10.1145/514188.514190},
  timestamp = {Tue, 06 Nov 2018 12:51:29 +0100},
  biburl    = {https://dblp.org/rec/journals/toplas/SagivRW02.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{ReifKIV,
author = {Reif, Wolfgang and Schellhorn, Gerhard and Stenzel, Kurt and Balser, Michael},
year = {2000},
month = {09},
pages = {},
title = {Structured Specifications and Interactive Proofs with KIV},
volume = {2},
isbn = {978-90-481-5051-9},
journal = {Automated Deduction - A Basis for Applications},
doi = {10.1007/978-94-017-0435-9_1}
}
